Understanding Visual Concepts Across Models

Large multimodal models such as Stable Diffusion can generate, detect, and classify new visual concepts after fine-tuning just a single word embedding. Do models learn similar words for the same concepts (i.e. <orange-cat> = orange + cat)? We conduct a large-scale analysis on three state-of-the-art models in text-to-image generation, open-set object detection, and zero-shot classification, and find that new word embeddings are model-specific and non-transferable. Across 4,800 new embeddings trained for 40 diverse visual concepts on four standard datasets, we find perturbations within an $\epsilon$-ball to any prior embedding that generate, detect, and classify an arbitrary concept. When these new embeddings are spliced into new models, fine-tuning that targets the original model is lost. We show popular soft prompt-tuning approaches find these perturbative solutions when applied to visual concept learning tasks, and embeddings for visual concepts are not transferable. Code for reproducing our work is available at: https://visual-words.github.io.

==> sections/checklist.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes
    \item[] Justification: Claims made in the abstract and introduction are grounded to the main experimental sections of the paper, including our section understanding when transfer fails using popular approaches for soft-prompt tuning, a section about perturbative solutions, and a section understanding what happens inside the model for non-transferable solutions.

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes
    \item[] Justification: We address potential limitations and risks associated with transferring soft prompts for visual concepts between models in the appendix of the submission.

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA
    \item[] Justification: This paper does not involve any theorems or proofs, and the inclusion of assumptions and correct proofs is not necessary, as the investigation presented in this work is empirical in nature and does not present on any new theory.

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes
    \item[] Justification: We have released open source code for our benchmark and methodology that fully reproduces the results in the paper, and have released a script that generates each evaluative figure in the paper. We have disclosed the configuration details for all models and datasets we used, and the experimental details in Section~\ref{sec:finding-one} used for optimizing word embeddings.

\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes
    \item[] Justification: We use open source datasets that are available for public download from their original sources, including ImageNet, COCO, PASCAL, and the DreamBooth dataset. We have described the steps taken to process these datasets to reproduce our results, and have released code for processing these datasets, and generate the results figures in this paper. 


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes
    \item[] Justification: We describe training, and testing datasets, and evaluation methodology in Section~\ref{sec:finding-one}. This sections discusses the hyperparameters used for optimizing new word embeddings, why these were chosen, and the open source code contains these choices, and can reproduce the results presented in this paper.

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes
    \item[] Justification: We report 95\% confidence intervals for all results in the paper, averaged over 100 independent randomized trials, which provides an accurate estimate on the confidence interval bounds. We employ the built-in seaborn (a popular Python plotting package based on matplotlib) confidence interval estimator, which in-turn uses scipy.

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes
    \item[] Justification: We discuss the computations requirements for each experiment in the Appendix. We employed an internal cluster of 40 2080ti GPUs, and run all models in float16 so that the larger models (Stable Diffusion 2.1, and OWL-v2) fit within an 11GB GPU. Each experiment requires less than 32GB of system RAM per trial, and when parallelized on 40 GPUs, takes less than 3 days of running to finish and generate all results in all sections of the paper. Section 4 takes 12 hours to run, Section 5 takes 2.5 days to run.
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes
    \item[] Justification: We discuss the potential ethical concerns that transferring soft prompts involves in the Appendix, and all experiments conform to the NeurIPS code of ethics. No human participants were involved in experiments in the paper, and all datasets used conform to the required levels of privacy and availability.

\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes
    \item[] Justification: We discuss both positive and negative potential broader impacts of transferring soft prompts for visual concepts between models in the Appendix of the manuscript.
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerYes
    \item[] Justification: We have discussed potential mitigation strategies that could be employed to safeguard the transfer of soft prompts between models in the Appendix.

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes
    \item[] Justification: We cite all models, datasets, and papers that influences this work, and have discussed the processing steps taken from these sources to reproduce the results in this paper. We use each model and dataset in a manner that adheres to the license of each.

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes
    \item[] Justification: We release open source code for processing data, training models, and reproducing all experiments in the paper. These assets are released alongside an MIT license, and an accompanying README that explains how to use the code to reproduce the paper.

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA
    \item[] Justification: No human subjects or crowd-sourced results are used in this paper, and this question is not applicable.

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA
    \item[] Justification: No human subjects or crowd-sourced results are used in this paper, and this question is not applicable.

\end{enumerate}
